On Coordinate Decoding for Keypoint Estimation Tasks

A series of 2D (and 3D) keypoint estimation tasks are built upon heatmap coordinate representation, i.e. a probability map that allows for learnable and spatially aware encoding and decoding of keypoint coordinates on grids, even allowing for sub-pixel coordinate accuracy. In this report, we aim to reproduce the findings of DARK that investigated the 2D heatmap representation by highlighting the importance of the encoding of the ground truth heatmap and the decoding of the predicted heatmap to keypoint coordinates. The authors claim that a) a more principled distribution-aware coordinate decoding method overcomes the limitations of the standard techniques widely used in the literature, and b), that the reconstruction of heatmaps from ground-truth coordinates by generating accurate and continuous heatmap distributions lead to unbiased model training, contrary to the standard coordinate encoding process that quantizes the keypoint coordinates on the resolution of the input image grid.

==> tables/human4d.tex <==

\begin{table}[ht]
\centering
\caption{Details with respect to the HUMAN4D physical, daily and social activities.}
\label{tbl::activities}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{clccc}
\toprule
            %& \textbf{id} 
            & \textbf{activity}
            %& \textbf{\# subjects} 
            %& \textbf{\# concurrent subjects} 
            & \textbf{\# frames} & \textbf{audio} & \textbf{type} \\
            \midrule
\parbox[t]{2mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{\textit{Single-person}}}}
%\textbf{1}  
& \textit{running}                                  
%& 4
%& 1
& 2,050                                     & \ourxmark                & physical                   \\
% & \textbf{2}  
& \textit{jumping\textunderscore jack}                                 %    & 4                                        & 1                                                   
& 1,974                                     & \ourxmark                & physical                   \\
%& \textbf{3}  
& \textit{bending}               %& 4                                        & 1                                                   
& 2,156                                       & \ourxmark              & physical                      \\
%& \textbf{4}  
& \textit{punching\textunderscore n\textunderscore kicking}                %& 4                                        & 1                                     
& 2,079                                       & \ourxmark                & physical                    \\
%& \textbf{5}  
& \textit{basketball\textunderscore dribbling}                         %     & 4                                        & 1  
& 2,124                                       & \ourxmark              & physical                     \\
%& \textbf{6}  
& \textit{laying\textunderscore down}                                  %     & 4                                        & 1
& 4,082                                       & \ourxmark                       & physical            \\
%& \textbf{7}  
& \textit{sitting\textunderscore down}            
%& 4                                        & 1
& 3,288                                       & \ourxmark                  & daily         \\
%& \textbf{8}  
& \textit{sitting\textunderscore on\textunderscore a\textunderscore chair}               %& 4                                        & 1
& 2,797                                       & \ourxmark           & daily                        \\
%& \textbf{9}  
& \textit{talking}                   
%& 4                                        & 1
& 2,377                                       & \checkmark                                 & daily  \\
%& \textbf{10} 
& \textit{object\textunderscore dropping\textunderscore n\textunderscore picking}       %& 4                                        & 1
&  1,768                                      & \ourxmark                        & daily           \\
%& \textbf{11} 
& \textit{stretching\textunderscore n\textunderscore talking}                          %& 4                                        & 1
&  2,787                                      & \checkmark                    & physical               \\
%& \textbf{12} 
& \textit{talking\textunderscore n\textunderscore walking} 
%& 4                                        & 1 
&  2,889                                      & \checkmark               & daily                    \\
%& \textbf{13} 
& \textit{watching\textunderscore scary\textunderscore movie}                     % & 4                                        & 1 
& 2,194                                       & \checkmark               & daily                    \\
%& \textbf{14} 
& \textit{in-flight\textunderscore safety\textunderscore announcement}                       %& 4                                        & 1
&  6,192                                      & \checkmark              &       daily               \\
\midrule
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{Multi-person}}}} %& \textbf{15} 
& \textit{watching\textunderscore football\textunderscore together}                        %& 4                                        & 2
&  1,760                                      & \checkmark          & social                         \\
%& \textbf{16} 
& \textit{dancing\textunderscore together}                                           %& 4                                        & 2 
& 1,356                                       & \checkmark            & social                         \\
%& \textbf{17} 
& \textit{physical\textunderscore examination}                              %& 4                                        & 2
& 2,328                                       & \checkmark           & social                          \\
%& \textbf{18} 
& \textit{whispering}               
%& 4                                        & 2
&  3,045                                      & \checkmark            & social                         \\
%& \textbf{19} 
& \textit{card\textunderscore trick}                           
%& 4                                        & 2
&  3,060                                      & \checkmark            & social        \\
\midrule
 %&                          &
 &                                                    &  50,306                                      &            &   \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/results_cont.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{+++++}
\begin{tabular}{@{}c|c|ccc@{}}
\toprule
\multicolumn{1}{l}{}                         & \textbf{Encoding}           & \multicolumn{1}{l}{\textbf{PCKh-0.1}} & \multicolumn{1}{l}{\textbf{PCKh-0.5}} & \multicolumn{1}{l}{\textbf{RMSE}} \\
\midrule
\multirow{8}{*}{StackedHourglass - 4 Stages} & \multirow{4}{*}{Quantized}  & 35.38                                 & 68.14                                 & 4.12                              \\
                                             &                             & 36.37                                 & 68.36                                 & 4.07                              \\
                                             &                             & 39.54                                 & 70.75                                 & 3.87                              \\
                                             &                             & 37.77                                 & 70.35                                 & 3.87                              \\
                                             & \multirow{4}{*}{Continuous} & 39.80                                 & 68.78                                 & 3.75                              \\
                                             &                             & 41.18                                 & 69.05                                 & 3.69                              \\
                                             &                             & \textbf{45.17}                        & \textbf{71.65}                        & 3.47                              \\
                                             &                             & 44.24                                 & 71.45                                 & \textbf{3.33}                     \\
                                             \midrule
\multirow{8}{*}{HRNet - 4 Stages}            & \multirow{4}{*}{Quantized}  & 37.29                                 & 68.10                                 & 3.93                              \\
                                             &                             & 38.48                                 & 68.35                                 & 3.87                              \\
                                             &                             & 41.73                                 & 70.29                                 & 3.65                              \\
                                             &                             & 33.95                                 & 68.38                                 & 3.94                              \\
                                             & \multirow{4}{*}{Continuous} & 39.19                                 & 68.60                                 & 3.85                              \\
                                             &                             & 40.50                                 & 68.90                                 & 3.79                              \\
                                             &                             & 44.83                                 & 71.52                                 & 3.55                              \\
                                             &                             & 36.77                                 & 70.21                                 & 3.79                  \\
                                             \bottomrule
\end{tabular}
\end{table}

==> tables/results_quant.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{+++++}
\begin{tabular}{@{}c|c|ccc@{}}
\toprule
\multicolumn{1}{l}{}                         & \textbf{Encoding}           & \multicolumn{1}{l}{\textbf{PCKh-0.1}} & \multicolumn{1}{l}{\textbf{PCKh-0.5}} & \multicolumn{1}{l}{\textbf{RMSE}} \\
\midrule
\multirow{8}{*}{StackedHourglass - 4 Stages} & \multirow{4}{*}{Quantized}  & 35.38                                 & 68.14                                 & 4.12                              \\
                                             &                             & 36.37                                 & 68.36                                 & 4.07                              \\
                                             &                             & 39.54                                 & 70.75                                 & 3.87                              \\
                                             &                             & 37.77                                 & 70.35                                 & 3.87                              \\
                                             & \multirow{4}{*}{Continuous} & 39.80                                 & 68.78                                 & 3.75                              \\
                                             &                             & 41.18                                 & 69.05                                 & 3.69                              \\
                                             &                             & \textbf{45.17}                        & \textbf{71.65}                        & 3.47                              \\
                                             &                             & 44.24                                 & 71.45                                 & \textbf{3.33}                     \\
                                             \midrule
\multirow{8}{*}{HRNet - 4 Stages}            & \multirow{4}{*}{Quantized}  & 37.29                                 & 68.10                                 & 3.93                              \\
                                             &                             & 38.48                                 & 68.35                                 & 3.87                              \\
                                             &                             & 41.73                                 & 70.29                                 & 3.65                              \\
                                             &                             & 33.95                                 & 68.38                                 & 3.94                              \\
                                             & \multirow{4}{*}{Continuous} & 39.19                                 & 68.60                                 & 3.85                              \\
                                             &                             & 40.50                                 & 68.90                                 & 3.79                              \\
                                             &                             & 44.83                                 & 71.52                                 & 3.55                              \\
                                             &                             & 36.77                                 & 70.21                                 & 3.79                  \\
                                             \bottomrule
\end{tabular}
\end{table}
